Parameterised algorithms for temporally satisfying reconfiguration problems

Given a static vertex-selection problem (e.g. independent set, dominating set) on a graph, we can define a corresponding temporally satisfying reconfiguration problem on a temporal graph which asks for a sequence of solutions to the vertex-selection problem at each time such that we can reconfigure from one solution to the next. We can think of each solution in the sequence as a set of vertices with tokens placed on them; our reconfiguration model allows us to slide tokens along active edges of a temporal graph at each time-step. We show that it is possible to efficiently check whether one solution can be reconfigured to another, and show that approximation results on the static vertex-selection problem can be adapted with a lifetime factor to the reconfiguration version. Our main contributions are fixed-parameter tractable algorithms with respect to: enumeration time of the related static problem; the combination of temporal neighbourhood diversity and lifetime of the input temporal graph; and the combination of lifetime and treewidth of the footprint graph.

==> sliding-dominating.tex <==

\section{Tree decomposition}

\subsection{Preliminaries}

\paragraph{Treewidth} A tree $T$ is a connected graph without a cycle. A tree decomposition of a static graph $G$ is a pair $(T, \mathcal{X})$ where $T$ is a tree and $\mathcal{X} = \{B_x \mid x \in V(T)\}$ is a collection of vertex subsets (called \emph{bags}), indexed by the nodes of $T$ such that:

\begin{compactenum}[(a)]
  \item for each edge $uv \in E(G)$, there is a bag $B_x$ containing $u$ and $v$ and,
  \item for each vertex $v \in V(G)$, the bags $B_x$ containing form a connected subset of $T$.
\end{compactenum}
The \emph{width} of the tree decomposition $(T,\mathcal{X})$ is defined to be $\max\{|B_x| \mid x \in V(T)\} -1$ and the treewidth of $G$ is the minimum value $k$ such that there is a tree decomposition of $G$ with width $k$.





%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "main"
%%% End:

